Disentangled representation learning for multilingual speaker recognition

The goal of this paper is to learn robust speaker representation for bilingual speaking scenario. The majority of the world's population speak at least two languages; however, most speaker recognition systems fail to recognise the same speaker when speaking in different languages. Popular speaker recognition evaluation sets do not consider the bilingual scenario, making it difficult to analyse the effect of bilingual speakers on speaker recognition performance. In this paper, we publish a large-scale evaluation set named VoxCeleb1-B derived from VoxCeleb that considers bilingual scenarios. We introduce an effective disentanglement learning strategy that combines adversarial and metric learning-based methods. This approach addresses the bilingual situation by disentangling language-related information from speaker representation while ensuring stable speaker representation learning. Our language-disentangled learning method only uses language pseudo-labels without manual information.

==> tab/exp_results.tex <==
\begin{table*}[t!]
\centering
\caption{Equal Error Rates (EER) and minimum Detection Cost Function (minDCF) on VoxCeleb1 test sets, VoxSRC validation sets and VoxCeleb1-B. 
All numbers are in percent (\%). 
All experiments are repeated three times, and we report the mean and the standard deviation.
{\bf Method}: Type of disentangled representation learning; COS and MAPC are cosine similarity and mean absolute Pearson's correlation minimisation. Ours is the gradient reversal with mean absolute Pearson's correlation minimisation.}
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c | c || c  c | c  c | c  c | c  c | c  c | c  c} 
\specialrule{.18em}{.05em}{.05em}
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method} & \multicolumn{2}{c|}{\bf VoxCeleb1 cl.} & \multicolumn{2}{c|}{\bf VoxCeleb1-E cl.} & \multicolumn{2}{c|}{\bf VoxCeleb1-H cl.} & \multicolumn{2}{c|}{\bf VoxSRC 2020 Val} & \multicolumn{2}{c|}{\bf VoxSRC 2021 Val} & \multicolumn{2}{c}{\bf VoxCeleb1-B}  \\
\cline{3-14}
& & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} \\
\specialrule{.18em}{.05em}{.05em}
\multirow{5}{*}{ResNet-S~\cite{chung2020defence}} & Baseline &  2.24~$\pm$~0.13 & 0.174~$\pm$~0.005 & 2.43~$\pm$~0.04 & 0.175~$\pm$~0.003 & 4.74~$\pm$~0.07 & 0.299~$\pm$~0.005 & 6.91~$\pm$~0.07 & 0.393~$\pm$~0.004 & 9.22~$\pm$~0.15 & 0.503~$\pm$~0.007 & 9.69~$\pm$~0.14 & 0.617~$\pm$~0.007 \\
\cline{2-14}
& GRL  & 2.98~$\pm$~0.14  & 0.210~$\pm$~0.012 & 3.12~$\pm$~0.19 & 0.222~$\pm$~0.013 & 5.72~$\pm$~0.37 & 0.351~$\pm$~0.020 & 8.07~$\pm$~0.47 & 0.457~$\pm$~0.025 & 10.27~$\pm$~0.88 & 0.541~$\pm$~0.036 & 10.39~$\pm$~1.24 & 0.598~$\pm$~0.055 \\
\cline{2-14}
& COS  & 2.13~$\pm$~0.08  & 0.164~$\pm$~0.006 & 2.45~$\pm$~0.06 & 0.178~$\pm$~0.004 & 4.78~$\pm$~0.12 & 0.303~$\pm$~0.006 & 6.83~$\pm$~0.06 & 0.388~$\pm$~0.004 & 9.33~$\pm$~0.18 & 0.505~$\pm$~0.002 & 10.21~$\pm$~0.22 & 0.614~$\pm$~0.012 \\
\cline{2-14}
& MAPC & 2.16~$\pm$~0.07  & 0.157~$\pm$~0.003 & 2.33~$\pm$~0.01 & 0.166~$\pm$~0.001 & 4.48~$\pm$~0.02 & 0.284~$\pm$~0.003 & 6.61~$\pm$~0.04 & 0.373~$\pm$~0.003 & 8.85~$\pm$~0.12 & 0.486~$\pm$~0.005 & 9.85~$\pm$~0.15 & 0.594~$\pm$~0.011 \\
\cline{2-14}
& Ours  & 2.15~$\pm$~0.01 & 0.172~$\pm$~0.001 & 2.42~$\pm$~0.01 & 0.171~$\pm$~0.00 & 4.49~$\pm$~0.02 & 0.284~$\pm$~0.001 & 6.54~$\pm$~0.02 & 0.378~$\pm$~0.001 & 8.35~$\pm$~0.05 & 0.461~$\pm$~0.002 & 8.25~$\pm$~0.06 & 0.506~$\pm$~0.002 \\

\specialrule{.18em}{.05em}{.05em}
\multirow{5}{*}{ResNet-L~\cite{kwon2021ins}} & Baseline &  1.17~$\pm$~0.00  & 0.083~$\pm$~0.003 & 1.30~$\pm$~0.01 & 0.091~$\pm$~0.001 & 2.58~$\pm$~0.02 & 0.164~$\pm$~0.001 & 4.06~$\pm$~0.02 & 0.231~$\pm$~0.005 & 5.16~$\pm$~0.08 & 0.308~$\pm$~0.010 & 5.96~$\pm$~0.23 & 0.397~$\pm$~0.016 \\
\cline{2-14}
& GRL & 1.22~$\pm$~0.04 & 0.088~$\pm$~0.009 & 1.34~$\pm$~0.04 & 0.096~$\pm$~0.002 & 2.58~$\pm$~0.02 & 0.166~$\pm$~0.001 & 4.13~$\pm$~0.04 & 0.230~$\pm$~0.003 & 4.53~$\pm$~0.25 & 0.263~$\pm$~0.008 & 3.98~$\pm$~0.27 & 0.268~$\pm$~0.020\\
\cline{2-14}
& COS  & 1.11~$\pm$~0.01 & 0.084$\pm$~0.007 & 1.25~$\pm$~0.03 & 0.091~$\pm$~0.004 & 2.52~$\pm$~0.02 & 0.164~$\pm$~0.002 & 3.99~$\pm$~0.03 & 0.228~$\pm$~0.002 & 5.21~$\pm$~0.18 & 0.317~$\pm$~0.015 & 5.99~$\pm$~0.35 & 0.423~$\pm$~0.016 \\
\cline{2-14}
& MAPC & 1.10~$\pm$~0.02 & 0.079~$\pm$~0.001 & 1.24~$\pm$~0.02 & 0.088~$\pm$~0.002 & 2.48~$\pm$~0.04 & 0.160~$\pm$~0.002 & 3.99~$\pm$~0.04 & 0.224~$\pm$~0.001 & 5.23~$\pm$~0.01 & 0.311~$\pm$~0.009 & 5.93~$\pm$~0.19 & 0.411~$\pm$~0.018 \\
\cline{2-14}
& Ours & 0.99~$\pm$~0.05 & 0.079~$\pm$~0.004 & 1.25~$\pm$~0.01 & 0.088~$\pm$~0.000 & 2.42~$\pm$~0.04 & 0.154~$\pm$~0.003 & 3.91~$\pm$~0.06 & 0.220~$\pm$~0.001 & 4.22~$\pm$~0.03 & 0.246~$\pm$~0.006 & 3.69~$\pm$~0.12 & 0.254~$\pm$~0.010 \\

\specialrule{.18em}{.05em}{.05em}
\end{tabular}}
\vspace{10pt}
\label{tab:results_main_old}
% \label{tab:results_main}
\end{table*}

% \begin{table*}[t!]
% \centering
% \caption{Equal Error Rates (EER) and minimum Detection Cost Function (minDCF) on VoxCeleb1 test sets, VoxSRC validation sets and VoxCeleb1-B. 
% All numbers are in percent (\%). 
% All experiments are repeated three times, and we report the mean and the standard deviation.
% {\bf Embed.}: Type of embedding method. Single stands for the single-embedding method and Multi stands for the multi-embedding method; {\bf Curr.}: Curriculum learning.}
% \renewcommand{\arraystretch}{1.2}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{c | c | c | c || c  c | c  c | c  c | c  c | c  c | c  c} 
% \specialrule{.18em}{.05em}{.05em}
% \multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Embed.} & \multirow{2}{*}{\bf $\lambda$} & \multirow{2}{*}{\bf Curr.} & \multicolumn{2}{c|}{\bf VoxCeleb1 cl.} & \multicolumn{2}{c|}{\bf VoxCeleb1-E cl.} & \multicolumn{2}{c|}{\bf VoxCeleb1-H cl.} & \multicolumn{2}{c|}{\bf VoxSRC 2020 Val} & \multicolumn{2}{c|}{\bf VoxSRC 2021 Val} & \multicolumn{2}{c}{\bf VoxCeleb1-B}  \\
% \cline{5-16}
% & & & & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} \\
% \specialrule{.18em}{.05em}{.05em}
% \multirow{9}{*}{ResNet-S~\cite{chung2020defence}} & Baseline & - & - & 2.24~$\pm$~0.13 & 0.174~$\pm$~0.005 & 2.43~$\pm$~0.04 & 0.175~$\pm$~0.003 & 4.74~$\pm$~0.07 & 0.299~$\pm$~0.005 & 6.91~$\pm$~0.07 & 0.393~$\pm$~0.004 & 9.22~$\pm$~0.15 & 0.503~$\pm$~0.007 & 9.69~$\pm$~0.14 & 0.617~$\pm$~0.007 \\
% \cline{2-16}
% & \multirow{4}{*}{Single} & \multirow{2}{*}{0.3} & \xmark & 2.52~$\pm$~0.04  & 0.190~$\pm$~0.003 & 2.68~$\pm$~0.11 & 0.194~$\pm$~0.007 & 5.10~$\pm$~0.19 & 0.323~$\pm$~0.011 & 7.26~$\pm$~0.26 & 0.420~$\pm$~0.015 & 9.34~$\pm$~0.38 & 0.500~$\pm$~0.016 & 9.16~$\pm$~0.42 & 0.550~$\pm$~0.032 \\
% & & & \cmark & 2.25~$\pm$~0.12  & 0.173~$\pm$~0.002 & 2.43~$\pm$~0.03 & 0.176~$\pm$~0.002 & 4.78~$\pm$~0.05 & 0.301~$\pm$~0.004 & 6.94~$\pm$~0.08 & 0.396~$\pm$~0.002 & 9.12~$\pm$~0.14 & 0.501~$\pm$~0.008 & 9.44~$\pm$~0.15 & 0.607~$\pm$~0.005 \\
% \cline{3-16}
% & & \multirow{2}{*}{0.5} & \xmark & 2.98~$\pm$~0.14  & 0.210~$\pm$~0.012 & 3.12~$\pm$~0.19 & 0.222~$\pm$~0.013 & 5.72~$\pm$~0.37 & 0.351~$\pm$~0.020 & 8.07~$\pm$~0.47 & 0.457~$\pm$~0.025 & 10.27~$\pm$~0.88 & 0.541~$\pm$~0.036 & 10.39~$\pm$~1.24 & 0.598~$\pm$~0.055 \\
% & & & \cmark & 2.24~$\pm$~0.11  & 0.175~$\pm$~0.004 & 2.43~$\pm$~0.03 & 0.177~$\pm$~0.002 & 4.78~$\pm$~0.06 & 0.302~$\pm$~0.004 & 6.96~$\pm$~0.08 & 0.398~$\pm$~0.004 & 8.95~$\pm$~0.10 & 0.495~$\pm$~0.008 & 9.19~$\pm$~0.16 & 0.595~$\pm$~0.006\\
% \cline{2-16}
% & \multirow{4}{*}{Multi} & \multirow{2}{*}{0.5} & \xmark & 2.53~$\pm$~0.05  & 0.191~$\pm$~0.003 & 2.71~$\pm$~0.02 & 0.197~$\pm$~0.002 & 5.04~$\pm$~0.05 & 0.320~$\pm$~0.001 & 7.23~$\pm$~0.06 & 0.417~$\pm$~0.003 & 7.63~$\pm$~0.17 & 0.447~$\pm$~0.001 & 6.50~$\pm$~0.12 & 0.444~$\pm$~0.013 \\
% & & & \cmark & 2.24~$\pm$~0.05 & 0.174~$\pm$~0.007 & 2.44~$\pm$~0.03 & 0.176~$\pm$~0.003 & 4.79~$\pm$~0.05 & 0.305~$\pm$~0.004 & 6.98~$\pm$~0.11 & 0.398~$\pm$~0.009 & 9.13~$\pm$~0.07 & 0.501~$\pm$~0.007 & 9.73~$\pm$~0.12 & 0.604~$\pm$~0.004\\
% \cline{3-16}
% & & \multirow{2}{*}{1.5} & \xmark & 3.71~$\pm$~0.03  & 0.267~$\pm$~0.006 & 3.76~$\pm$~0.05 & 0.269~$\pm$~0.002 & 5.93~$\pm$~0.11 & 0.373~$\pm$~0.010 & 8.21~$\pm$~0.15 & 0.486~$\pm$~0.007 & 6.90~$\pm$~0.22 & 0.440~$\pm$~0.013 & 4.91~$\pm$~0.28 & 0.371~$\pm$~0.027 \\
% & & & \cmark & 2.22~$\pm$~0.05 & 0.171~$\pm$~0.008 & 2.45~$\pm$~0.04 & 0.180~$\pm$~0.004 & 4.82~$\pm$~0.07 & 0.310~$\pm$~0.005 & 7.00~$\pm$~0.11 & 0.403~$\pm$~0.010 & 7.93~$\pm$~0.22 & 0.460~$\pm$~0.014 & 7.65~$\pm$~0.38 & 0.516~$\pm$~0.021\\
% \specialrule{.18em}{.05em}{.05em}
% \multirow{9}{*}{ResNet-L~\cite{kwon2021ins}} & Baseline & - & - & 1.17~$\pm$~0.00  & 0.083~$\pm$~0.003 & 1.30~$\pm$~0.01 & 0.091~$\pm$~0.001 & 2.58~$\pm$~0.02 & 0.164~$\pm$~0.001 & 4.06~$\pm$~0.02 & 0.231~$\pm$~0.005 & 5.16~$\pm$~0.08 & 0.308~$\pm$~0.010 & 5.96~$\pm$~0.23 & 0.397~$\pm$~0.016 \\
% \cline{2-16}
% & \multirow{4}{*}{Single} & \multirow{2}{*}{0.5} & \xmark & 1.22~$\pm$~0.04 & 0.088~$\pm$~0.009 & 1.34~$\pm$~0.04 & 0.096~$\pm$~0.002 & 2.58~$\pm$~0.02 & 0.166~$\pm$~0.001 & 4.13~$\pm$~0.04 & 0.230~$\pm$~0.003 & 4.53~$\pm$~0.25 & 0.263~$\pm$~0.008 & 3.98~$\pm$~0.27 & 0.268~$\pm$~0.020\\
% & & & \cmark & \textbf{1.12~$\pm$~0.02} & \textbf{0.083~$\pm$~0.000} & \textbf{1.30~$\pm$~0.01} & \textbf{0.091~$\pm$~0.001} & \textbf{2.56~$\pm$~0.01} & \textbf{0.164~$\pm$~0.001} & \textbf{4.04~$\pm$~0.01} & \textbf{0.229~$\pm$~0.005} & 4.87~$\pm$~0.04 & 0.290~$\pm$~0.007 & 5.19~$\pm$~0.17 & 0.348~$\pm$~0.014\\
% \cline{3-16}
% & & \multirow{2}{*}{1.5} & \xmark & 1.75~$\pm$~0.06 & 0.126~$\pm$~0.006 & 1.80~$\pm$~0.01 & 0.122~$\pm$~0.002 & 2.87~$\pm$~0.05 & 0.178~$\pm$~0.006 & 4.40~$\pm$~0.05 & 0.249~$\pm$~0.004 & \textbf{3.98~$\pm$~0.13} & \textbf{0.233~$\pm$~0.001} & \textbf{3.08~$\pm$~0.20} & \textbf{0.215~$\pm$~0.007} \\
% & & & \cmark & 1.48~$\pm$~0.08 & 0.101~$\pm$~0.005 & 1.58~$\pm$~0.03 & 0.107~$\pm$~0.001 & 2.63~$\pm$~0.02 & 0.166~$\pm$~0.001 & 4.09~$\pm$~0.02 & 0.230~$\pm$~0.003 & 4.89~$\pm$~0.19 & 0.274~$\pm$~0.011 & 4.62~$\pm$~0.31 & 0.309~$\pm$~0.020 \\
% \cline{2-16}
% & \multirow{4}{*}{Multi} & \multirow{2}{*}{0.5} & \xmark & 1.28~$\pm$~0.03 & 0.095~$\pm$~0.001 & 1.41~$\pm$~0.01 & 0.100~$\pm$~0.000 & 2.69~$\pm$~0.02 & 0.172~$\pm$~0.000 & 4.23~$\pm$~0.03 & 0.239~$\pm$~0.001 & 5.09~$\pm$~0.10 & 0.303~$\pm$~0.007 & 5.17~$\pm$~0.08 & 0.356~$\pm$~0.004 \\
% & & & \cmark & 1.21~$\pm$~0.03 & 0.088~$\pm$~0.005 & 1.32~$\pm$~0.01 & 0.092~$\pm$~0.002 & 2.60~$\pm$~0.01 & 0.165~$\pm$~0.002 & 4.11~$\pm$~0.01 & 0.231~$\pm$~0.003 & 5.21~$\pm$~0.06 & 0.308~$\pm$~0.005 & 5.87~$\pm$~0.19 & 0.387~$\pm$~0.007 \\
% \cline{3-16}
% & & \multirow{2}{*}{1.5} & \xmark & 1.78~$\pm$~0.06 & 0.129~$\pm$~0.006 & 1.77~$\pm$~0.05 & 0.127~$\pm$~0.005 & 3.20~$\pm$~0.07 & 0.205~$\pm$~0.010 & 4.85~$\pm$~0.10 & 0.280~$\pm$~0.011 & 4.42~$\pm$~0.30 & 0.268~$\pm$~0.017 & 3.33~$\pm$~0.50 & 0.234~$\pm$~0.032 \\
% & & & \cmark & 1.23~$\pm$~0.03 & 0.091~$\pm$~0.002 & 1.34~$\pm$~0.01 & 0.093~$\pm$~0.003 & 2.59~$\pm$~0.03 & 0.164~$\pm$~0.003 & 4.10~$\pm$~0.03 & 0.230~$\pm$~0.002 & 5.04~$\pm$~0.06 & 0.301~$\pm$~0.010 & 5.47~$\pm$~0.18 & 0.371~$\pm$~0.008\\

% \specialrule{.18em}{.05em}{.05em}
% \end{tabular}}
% \vspace{10pt}
% \label{tab:results_main}
% \end{table*}

==> tab/exp_results_CL.tex <==
\begin{table*}[t!]
\centering
\caption{Equal Error Rates (EER) and minimum Detection Cost Function (minDCF) on VoxSRC 2021 validation set and VoxCeleb1-B. 
All numbers are in percent (\%). 
All experiments are repeated three times, and we report the mean and the standard deviation.}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{c | c || c  c | c  c } 
\specialrule{.18em}{.05em}{.05em}
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method} & \multicolumn{2}{c|}{\bf VoxSRC 2021 Val} & \multicolumn{2}{c}{\bf VoxCeleb1-B}  \\
\cline{3-6}
& & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} \\
\specialrule{.18em}{.05em}{.05em}
\multirow{5}{*}{ResNet-S} & Baseline &  9.22~$\pm$~0.15 & 0.503~$\pm$~0.007 & 9.69~$\pm$~0.14 & 0.617~$\pm$~0.007 \\
% \cline{2-6}
& GRL  & 10.27~$\pm$~0.88 & 0.541~$\pm$~0.036 & 10.39~$\pm$~1.24 & 0.598~$\pm$~0.055 \\
% \cline{2-6}
& COS  & 9.33~$\pm$~0.18 & 0.505~$\pm$~0.002 & 10.21~$\pm$~0.22 & 0.614~$\pm$~0.012 \\
% \cline{2-6}
& MAPC & 8.85~$\pm$~0.12 & 0.486~$\pm$~0.005 & 9.85~$\pm$~0.15 & 0.594~$\pm$~0.011 \\
% \cline{2-6}
& Ours & 8.35~$\pm$~0.05 & 0.461~$\pm$~0.002 & 8.25~$\pm$~0.06 & 0.506~$\pm$~0.002 \\

\specialrule{.18em}{.05em}{.05em}
\multirow{5}{*}{ResNet-L} & Baseline & 5.16~$\pm$~0.08 & 0.308~$\pm$~0.010 & 5.96~$\pm$~0.23 & 0.397~$\pm$~0.016 \\
% \cline{2-6}
& GRL & 4.53~$\pm$~0.25 & 0.263~$\pm$~0.008 & 3.98~$\pm$~0.27 & 0.268~$\pm$~0.020\\
% \cline{2-6}
& COS & 5.21~$\pm$~0.18 & 0.317~$\pm$~0.015 & 5.99~$\pm$~0.35 & 0.423~$\pm$~0.016 \\
% \cline{2-6}
& MAPC & 5.23~$\pm$~0.01 & 0.311~$\pm$~0.009 & 5.93~$\pm$~0.19 & 0.411~$\pm$~0.018 \\
% \cline{2-6}
& Ours & 4.22~$\pm$~0.03 & 0.246~$\pm$~0.006 & 3.69~$\pm$~0.12 & 0.254~$\pm$~0.010 \\

\specialrule{.18em}{.05em}{.05em}
\end{tabular}}
\vspace{10pt}
\label{tab:results_CL}
\end{table*}

==> tab/exp_results_existing.tex <==
\begin{table*}[t!]
\centering
\caption{Equal Error Rates (EER) and minimum Detection Cost Function (minDCF) on VoxCeleb1 test sets and VoxSRC 2020 validation set. 
All numbers are in percent (\%). 
All experiments are repeated three times, and we report the mean and the standard deviation.
{\bf Method}: Type of disentangled representation learning; COS and MAPC are cosine similarity and mean absolute Pearson's correlation minimisation. Ours is the gradient reversal with mean absolute Pearson's correlation minimisation.}
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c | c || c  c | c  c | c  c | c  c} 
\specialrule{.18em}{.05em}{.05em}
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method} & \multicolumn{2}{c|}{\bf VoxCeleb1 cl.} & \multicolumn{2}{c|}{\bf VoxCeleb1-E cl.} & \multicolumn{2}{c|}{\bf VoxCeleb1-H cl.} & \multicolumn{2}{c}{\bf VoxSRC 2020 Val}  \\
\cline{3-10}
& & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} & {\bf EER} & {\bf minDCF} \\
\specialrule{.18em}{.05em}{.05em}
\multirow{5}{*}{ResNet-S~\cite{chung2020defence}} & Baseline &  2.24~$\pm$~0.13 & 0.174~$\pm$~0.005 & 2.43~$\pm$~0.04 & 0.175~$\pm$~0.003 & 4.74~$\pm$~0.07 & 0.299~$\pm$~0.005 & 6.91~$\pm$~0.07 & 0.393~$\pm$~0.004  \\
% \cline{2-10}
& GRL  & 2.98~$\pm$~0.14  & 0.210~$\pm$~0.012 & 3.12~$\pm$~0.19 & 0.222~$\pm$~0.013 & 5.72~$\pm$~0.37 & 0.351~$\pm$~0.020 & 8.07~$\pm$~0.47 & 0.457~$\pm$~0.025  \\
% \cline{2-10}
& COS  & 2.13~$\pm$~0.08  & 0.164~$\pm$~0.006 & 2.45~$\pm$~0.06 & 0.178~$\pm$~0.004 & 4.78~$\pm$~0.12 & 0.303~$\pm$~0.006 & 6.83~$\pm$~0.06 & 0.388~$\pm$~0.004  \\
% \cline{2-10}
& MAPC & 2.16~$\pm$~0.07  & 0.157~$\pm$~0.003 & 2.33~$\pm$~0.01 & 0.166~$\pm$~0.001 & 4.48~$\pm$~0.02 & 0.284~$\pm$~0.003 & 6.61~$\pm$~0.04 & 0.373~$\pm$~0.003  \\
% \cline{2-10}
& Ours  & 2.15~$\pm$~0.01 & 0.172~$\pm$~0.001 & 2.42~$\pm$~0.01 & 0.171~$\pm$~0.00 & 4.49~$\pm$~0.02 & 0.284~$\pm$~0.001 & 6.54~$\pm$~0.02 & 0.378~$\pm$~0.001 \\

\specialrule{.18em}{.05em}{.05em}
\multirow{5}{*}{ResNet-L~\cite{kwon2021ins}} & Baseline &  1.17~$\pm$~0.00  & 0.083~$\pm$~0.003 & 1.30~$\pm$~0.01 & 0.091~$\pm$~0.001 & 2.58~$\pm$~0.02 & 0.164~$\pm$~0.001 & 4.06~$\pm$~0.02 & 0.231~$\pm$~0.005 \\
% \cline{2-10}
& GRL & 1.22~$\pm$~0.04 & 0.088~$\pm$~0.009 & 1.34~$\pm$~0.04 & 0.096~$\pm$~0.002 & 2.58~$\pm$~0.02 & 0.166~$\pm$~0.001 & 4.13~$\pm$~0.04 & 0.230~$\pm$~0.003 \\
% \cline{2-10}
& COS  & 1.11~$\pm$~0.01 & 0.084$\pm$~0.007 & 1.25~$\pm$~0.03 & 0.091~$\pm$~0.004 & 2.52~$\pm$~0.02 & 0.164~$\pm$~0.002 & 3.99~$\pm$~0.03 & 0.228~$\pm$~0.002  \\
% \cline{2-10}
& MAPC & 1.10~$\pm$~0.02 & 0.079~$\pm$~0.001 & 1.24~$\pm$~0.02 & 0.088~$\pm$~0.002 & 2.48~$\pm$~0.04 & 0.160~$\pm$~0.002 & 3.99~$\pm$~0.04 & 0.224~$\pm$~0.001  \\
% \cline{2-10}
& Ours & 0.99~$\pm$~0.05 & 0.079~$\pm$~0.004 & 1.25~$\pm$~0.01 & 0.088~$\pm$~0.000 & 2.42~$\pm$~0.04 & 0.154~$\pm$~0.003 & 3.91~$\pm$~0.06 & 0.220~$\pm$~0.001  \\

\specialrule{.18em}{.05em}{.05em}
\end{tabular}}
\vspace{10pt}
\label{tab:results_existing}
\end{table*}

==> tab/exp_slr_results.tex <==
\begin{table}[t]
\caption{Equal Error Rates (EER) and Language Classification Accuracy on VoxCeleb1-B. SPK and SLR stand for the task of speaker recognition and language recognition. All numbers are in percent (\%).}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c |c |  c| c } 

\specialrule{.13em}{.05em}{.05em}
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method} &   {\bf VoxCeleb1-B SPK} & {\bf VoxCeleb1-B SLR} \\
\cline{3-4}
 &  &  EER & Accuracy \\
\specialrule{.13em}{.05em}{.05em}
\multirow{4.5}{*}{ResNet-L} & Baseline &  5.96~$\pm$~0.23 & 88.3 \\
% \cline{2-4}
& GRL &   3.98~$\pm$~0.27 & 72.1 \\
% \cline{2-4}
& COS &  5.99~$\pm$~0.35 & - \\
% \cline{2-4}
& MAPC &  5.93~$\pm$~0.19 & - \\
% \cline{2-4}
& GRPC &  3.69~$\pm$~0.12 & - \\

\specialrule{.13em}{.05em}{.05em}
\end{tabular}}
\label{tab:results_extra}
\end{table}

==> tab/new_exp_slr_results.tex <==
\begin{table}[t]
\centering
\caption{Equal Error Rates (EER) and Language Classification Accuracy on VoxCeleb1-B. SPK and SLR stand for the task of speaker recognition and language recognition. All numbers are in percent (\%).}
\resizebox{0.8\linewidth}{!}{\begin{tabular}{c |c |  c| c } 

\specialrule{.13em}{.05em}{.05em}
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method} &   {\bf SPK} & {\bf SLR} \\
\cline{3-4}
 &  &  EER & Accuracy \\
\specialrule{.13em}{.05em}{.05em}
\multirow{4.5}{*}{ResNet-L} & Baseline &  5.96~$\pm$~0.23 & 88.3 \\
% \cline{2-4}
& GRL &   3.98~$\pm$~0.27 & 72.1 \\
% \cline{2-4}
& COS &  5.99~$\pm$~0.35 & - \\
% \cline{2-4}
& MAPC &  5.93~$\pm$~0.19 & - \\
% \cline{2-4}
& GRPC &  3.69~$\pm$~0.12 & - \\

\specialrule{.13em}{.05em}{.05em}
\end{tabular}}
\label{tab:results_extra}
\end{table}

==> tab/old_test_sets.tex <==
\begin{table*}[t!]
\centering
\caption{Statistics of the VoxCeleb1 test sets, VoxSRC validation sets and VoxCeleb1-B. {\bf Pos.}: \# of positive trials; {\bf Neg.}: \# of negative trials; {\bf cl.}: Cleaned version of the test set; {\bf Cross-lingual}: \kyk{Whether to contain} a significant number of cross-lingual positive pairs.}
\vspace{-2mm}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{\extracolsep{8pt}}lcccccccccccc@{}}
% c |cc|cc|cc|cc|cc|cc} 
% \specialrule{.1em}{.05em}{.05em}
\toprule
\multirow{2}{*}{\bf test set}            & \multicolumn{2}{c}{\bf VoxCeleb1 cl.} & \multicolumn{2}{c}{\bf VoxCeleb1-E cl.} & \multicolumn{2}{c}{\bf VoxCeleb1-H cl.} & \multicolumn{2}{c}{\bf VoxSRC 2020 Val} & \multicolumn{2}{c}{\bf VoxSRC 2021 Val} & \multicolumn{2}{c}{\bf VoxCeleb1-B}  \\
\cmidrule[0.2pt]{2-3} \cmidrule[0.2pt]{4-5} \cmidrule[0.2pt]{6-7} \cmidrule[0.2pt]{8-9} \cmidrule[0.2pt]{10-11} \cmidrule[0.2pt]{12-13}
& {\bf Pos.} & {\bf Neg.} & {\bf Pos.} & {\bf Neg.} & {\bf Pos.} & {\bf Neg.} & {\bf Pos.} & {\bf Neg.} & {\bf Pos.} & {\bf Neg.} & {\bf Pos.} & {\bf Neg.} \\
% \specialrule{.1em}{.05em}{.05em}
\toprule
\# of pairs & 18,860 & 18,860 & 289,921 & 289,897 & 275,488 & 275,406 & 131,743 & 131,743 & 29,969 & 30,031 & 404,287 & 404,287\\
% \# of hard pairs & 1,289 & 16,454 & 10,638 & 265,987 & 7,655 & 264,025 & 4,049 & 126,876 & 17,957 & 29,551 & 404,287 & 404,287\\

total \# of pairs  & \multicolumn{2}{c}{37,720 (18,860 / 18,860)}     &  \multicolumn{2}{c}{579,818}  & \multicolumn{2}{c}{550,894}  &  \multicolumn{2}{c}{263,486} & \multicolumn{2}{c}{60,000} &  \multicolumn{2}{c}{808,574}           \\

Cross-lingual  & \multicolumn{2}{c}{\xmark}     &  \multicolumn{2}{c}{\xmark}  & \multicolumn{2}{c}{\xmark}  &  \multicolumn{2}{c}{\xmark} & \multicolumn{2}{c}{\cmark} &  \multicolumn{2}{c}{\cmark}           \\
% \specialrule{.1em}{.05em}{.05em}
\bottomrule
\end{tabular}}

\label{tab:testsets}
\end{table*}
